Continuous Assortment Optimization with Logit Choice Probabilities under Incomplete Information

We consider assortment optimization over a continuous spectrum of products represented by the unit interval, where the seller's problem consists of determining the optimal subset of products to offer to potential customers. To describe the relation between assortment and customer choice, we propose a probabilistic choice model that forms the continuous counterpart of the widely studied discrete multinomial logit model. We consider the seller's problem under incomplete information, propose a stochastic-approximation type of policy, and show that its regret -- its performance loss compared to the optimal policy -- is only logarithmic in the time horizon. We complement this result by showing a matching lower bound on the regret of any policy, implying that our policy is asymptotically optimal. We then show that adding a capacity constraint significantly changes the structure of the problem: we construct a policy and show that its regret after $T$ time periods is bounded above by a constant times $T^{2/3}$ (up to a logarithmic term); in addition, we show that the regret of any policy is bounded from below by a positive constant times $T^{2/3}$, so that also in the capacitated case we obtain asymptotic optimality. Numerical illustrations show that our policies outperform or are on par with alternatives.

==> nieuw6.tex <==
\section{Numerical experiments}
\label{sec:numerical}

\iffalse
\subsection{Application to static assortment optimization with mortgage loan data}

We first demonstrate the use of our continuous multinomial logit choice model and estimator of the preference function on the {\it Single-Family Loan Performance Dataset} from the Federal National Mortgage Association (FNMA). Founded in 1938, the FNMA is one of the largest corporations in the US with a reported net income of about \$1.6 billion in 2018.

The entire loan dataset contains the acquisition of single-family, conventional fixed-rate mortgages from the first quarter of 2000 until the third quarter of 2018. The full dataset being extremely large, we chose to focus on the loans approved of in the third quarter of 2018 with a pay-off term of 30 years, covering over $380\,000$ observations. Figure \ref{fig:histogram} shows a histogram of the loan amounts. We scale the loans in the computations with the maximum loan in the dataset (i.e., $\$800\,000$), so that the product set becomes $[0,1]$.

The dataset does not contain records of no-purchases. To assess the sensitivity of the outcomes in the value of the no-purchase probability, we determine the optimal assortment for different values of this probability. In practice, one could provide an estimate of this probability by e.g.,\ considering additional purchase data or market share estimates.

Furthermore, corresponding to a setting that does not take into account changes in the interest rate, we let the marginal profit function be a linear function of the amount of the loan. More specifically, re-scaling the marginal profit function appropriately, we consider 
$w(x) = x$, for all $x \in [0,1]$. 
We use the KDE technique from Section \ref{sec:capacitated} to estimate the preference function, and compute the corresponding optimal assortment without capacity constraints for different choices of the no-purchase probability. 

Table \ref{T1} summarizes the results of the computations. In line with our theoretical findings, the optimal assortment consists of only offering loans beyond a certain minimum value. In addition, it shows that the profit gain compared to offering all loan sizes is 2 to 6 percent, depending on the no-purchase probability. This suggests that in applications that involve a continuous product space, profits may be significantly increased by estimating the preference function and using the corresponding optimal assortment instead of offering the whole product range. 

\begin{figure}[h!]
\begin{centering}
\begin{minipage}{\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
  ymin=0, ymax=60000,
 	xmin=0,xmax=800000,
 	ylabel=Frequency,
 	xlabel=Loan amount \vphantom{\Big|},
  minor y tick num = 4,
  xtick scale label code/.code={$\times 10^5$},
  ytick scale label code/.code={$\times 10^4$}
  ]
\addplot+[ybar interval,mark=no,fill=gray!50,draw=black] plot coordinates { (0, 998) (40000, 16758) (80000, 38190) (120000, 49817) (160000, 51455) (200000, 53301) (240000, 42781) (280000, 35102) (320000, 27365) (360000, 21040) (400000, 17408) (440000, 14830) (480000, 3988) (520000, 2999) (560000, 2358) (600000, 2041) (640000, 2011) (680000, 864) (720000, 71) (760000, 46) };
\end{axis}
\end{tikzpicture}
\end{minipage}
\caption{Histogram of the loan amounts of single-family, conventional fixed-rate mortgages granted by the FNMA in the third quarter of 2018.}
\label{fig:histogram}
\end{centering}
\end{figure}

\begin{table}[h!]
  \centering
    \begin{tabular}{|c|c|c|}
      \hline\hline
      No-purchase probability & Optimal assortment & Relative profit gain \vphantom{\Big|}\\
      \hline
       $p=0.5$ & $\geqslant \$166\,070$ & $6.08\%$ \\
       $p=0.6$ & $\geqslant \$152\,799$ & $4.58\%$ \\
       $p=0.7$ & $\geqslant \$141\,800$ & $3.52\%$ \\
       $p=0.8$ & $\geqslant \$132\,471$ & $2.75\%$ \\
       $p=0.9$ & $\geqslant \$124\,415$ & $2.18\%$ \\
       \hline\hline
    \end{tabular}\vspace{3mm}
  \caption{\label{T1}Summary of the results of the numerical study on loan data.}
\end{table}
\fi

%\subsection{Numerical comparison to discretization-based approaches}

In this section we compare the numerical performance of the policies proposed in this work to alternatives that are based on discretizing the product space and subsequently applying an algorithm designed for discrete assortment optimization under the discrete multinomial logit (MNL) model. We use the notations and concepts introduced in Sections \ref{sec:capacitatedpolicy} and \ref{sec:capacitatedupperbound}. The procedure of discretization used for DUCB is also used for the discrete policies we compare here. We compare the two algorithms proposed in this paper to the Thompson Sampling based algorithm by \cite{Agrawal2017}, and (for the uncapacitated case) the Trisection based algorithm by \cite{Chen2018}. We refer to the policies with the added discretization procedure with as Discretized Thompson Sampling (DTS) and Discretized Trisection (DTR), respectively. We set the preference function $v$ as the bi-modal function that is plotted in Figure \ref{fig:simulationv}. This function is defined as
\begin{equation}
  v(x) = \frac{1}{10}+\frac{1}{5}(2+x)(1-x) + \frac{2}{7}\phi(x;0.33,0.1) + \frac{1}{5}\phi(x;0.8,0.1), \qquad x\in[0,1],
  \label{eq:simv2}
\end{equation}
where $\phi(\,\cdot\,;\mu,\sigma)$ denotes the normal probability density function with mean $\mu$ and standard deviation $\sigma$. In addition, we set
$w(x) = x$, $x\in[0,1]$, as the marginal profit function. The DTS algorithm is implemented with capacity constraint $K = N$ (i.e.,\ no capacity constraint) and $K = \floor{0.5N}$ (corresponding to $c = 0.5$); the DTR algorithm is only implemented without capacity constraint. We record the algorithms' average regret over 100 simulations after $T$ time periods, for $T \in \{1\,000, 2\,000, \ldots, 10\,000\}$. Then, in line with Theorem \ref{th:upperboundc<1} we set the discretization parameter $N$ as $\floor{\gamma T^{1/3}}$ with $\gamma = \max\{\vmax,1/c+1\}$ and $\vmax = 2$. For the case of $c =1$, we compare the performances of DTS, DTR, DUCB and SAP (with parameters $\alpha = 3$, $\beta = 2$, $\varrho_1 = 0$). For the case of $c = 0.5$ we compare the performance of DTS and DUCB. The results are reported in Table \ref{tab:T2} and \ref{tab:T3}. For each algorithm, we have included the maximum relative standard error (MRSE), where the maximum is taken over values of $T \in \{1\,000, 2\,000, \ldots, 10\,000\}$. In addition, we simulate the regret for Adjusted DUCB (ADUCB). For this algorithm we replace $48$ in \eqref{eq:updatevUCB} with $1$. Besides the average regret over 100 simulations we compute the loss due to discretization. In general, the best achievable assortment after discretization with parameter $N$ is contained in
\[\max_{S\in\mathcal{A}_K} r(S,v),\]
where $K=\floor{cN}$ and $\mathcal{A}_K$ is as in \eqref{eq:setofbincollections}. Then, we refer to the difference between the optimal expected profit and the best achievable expected profit as discretization loss, that is,
\[DL := \max_{S\in\cS} r(S,v) - \max_{S\in\mathcal{A}_K} r(S,v).\]

The results show that our algorithm SAP significantly outperforms the four alternatives (DTR, DTS, DUCB and ADUCB) in the uncapacitated setting. In the capacitated setting, the adjusted policy ADUCB performs on par with DTS. Both ADUCB and DTS outperform the unadjusted policy DUCB. This suggests that fine-tuning the constants in the updating formula for the upper confidence bounds can lead to less regret. Interestingly, the regret for DTS and ADUCB sometimes seems to dip for increasing values of $T$. We note that all these dips occur when a sudden dip of discretization loss also occurs.

\begin{table}[H]
  \centering
  \small
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
      \hline\hline
       & \multicolumn{11}{c|}{Time horizon $T$}\\
      \hline
      Policy & 1\,000 & 2\,000 & 3\,000 & 4\,000 & 5\,000 & 6\,000 & 7\,000 & 8\,000 & 9\,000 & 10\,000 & MRSE \vphantom{\Big|}\\
      \hline
       DTR & 8.67 & 18.2 & 25.5 & 32.1 & 35.9 & 40.9 & 48.3 & 55.8 & 63.7 & 70.0 & 0.44\% \\
       DTS & 1.46 & 1.94 & 2.10 & 2.25 & 2.56 & 2.45 & 2.87 & 3.06 & 2.85 & 3.34 & 2.6\% \\
       DUCB & 95.9 & 172 & 235 & 297 & 357 & 412 & 467 & 515 & 567 & 620 & 0.099\% \\
       ADUCB & 11.9 & 19.1 & 23.5 & 28.1 & 32.8 & 35.3 & 38.4 & 41.0 & 43.1 & 46.9 & 1.2\% \\
       SAP & 0.380 & 0.417 & 0.439 & 0.452 & 0.463 & 0.474 & 0.483 & 0.49 & 0.500 & 0.507 & 3.4\% \\
       \hline
       $N$ & 19 & 25 & 28 & 31 & 34 & 36 & 38 & 39 & 41 & 43 & \\
       $DL\times 10^5$ & 1.90 & 9.84 & 0.53 & 1.78 & 4.69 & 0.463 & 1.90 & 5.10 & 0.0372 & 2.52 & \\
       \hline\hline
    \end{tabular}\vspace{3mm}
  \caption{\label{tab:T2} Simulated average regret of the policies with $c = 1$ based on 100 simulations.}
\end{table}

\begin{table}[H]
  \centering
  \small
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
      \hline\hline
       & \multicolumn{11}{c|}{Time horizon $T$}\\
      \hline
      Policy & 1\,000 & 2\,000 & 3\,000 & 4\,000 & 5\,000 & 6\,000 & 7\,000 & 8\,000 & 9\,000 & 10\,000 & MRSE \vphantom{\Big|}\\
      \hline
       DTS & 12.8 & 19.8 & 26.8 & 32.0 & 38.8 & 33.2 & 46.8 & 52.6 & 43.8 & 48.0 & 2.1\% \\
       DUCB & 89.6 & 153 & 206 & 252 & 295 & 334 & 371 & 403 & 440 & 470 & 0.13\% \\
       ADUCB & 9.81 & 16.9 & 23.6 & 29.8 & 35.3 & 32.6 & 46.7 & 52.1 & 45.8 & 50.1 & 0.68\% \\
       \hline
       $N$ & 29 & 37 & 43 & 47 & 51 & 54 & 57 & 59 & 62 & 64 &  \\
       $DL\times 10^3$ & 2.93 & 2.19 & 1.80 & 1.72 & 1.49 & 0.0179 & 1.34 & 1.33 & 0.0730 & 0.480 & \\
       \hline\hline
    \end{tabular}\vspace{3mm}
  \caption{\label{tab:T3} Simulated average regret of the policies with $c=0.5$ based on 100 simulations.}
\end{table}

Lastly, we illustrate the growth rate of the regret that we found in the previous sections. More concretely, using ordinary least squares we fit the simulated regret of SAP to the curve
\[K_1(T)=\gamma_1\log T + \gamma_2,\]
and we fit the simulated regret of DUCB and ADUCB to the curve
\[K_2(T)= \gamma_1\:T^{2/3} + \gamma_2.\]
% For a reliable fit, we increase the number of simulations to 1\,000 for each value of $T\in\{1\,000, 2\,000, \ldots, 10\,000\}$. 
As is shown in Figure \ref{fig:regression}, for each value of $T\in\{1\,000, 2\,000, \ldots, 10\,000\}$, we find that the 95\% confidence intervals of the mean regret of SAP contain the values of the corresponding fitted curve $K_1$. For the mean regret of DUCB the fitted curve $K_2$ mostly follow the bounds of the confidence intervals. For ADUCB the effect of the discretization loss is more profound and, as a result, the mean regret does not seem to behave as a smooth function of $T$.

\begin{figure}[H]
\begin{center}
\begin{tikzpicture}
\begin{axis}[
  width = 0.45\linewidth,
  xmin = 0, xmax = 10000,
  ymin = 0,
  xtick={2000,4000,6000,8000,10000},
  xticklabels={$2$,$4$,$6$,$8$,$10$},
  xtick scale label code/.code={$\times 10^4$},
  xlabel={$T$},
  ylabel={$\reg(T)$},
  legend pos = south east,
]

\addplot[
	black,
	only marks,
	mark = triangle*,
	mark options={rotate=60,scale=0.8,fill=gray},]
  table {UCB1.dat};
\addlegendentry{\footnotesize UCB}

\addplot[
	black,
	only marks,
	mark = triangle*,
	mark options={scale=0.8,fill=gray},]
  table {LCB1.dat};
\addlegendentry{\footnotesize LCB}

\addplot[
	smooth,
  solid,
  color=blue,
  domain=3:10000,
  samples=1000,
  ]
  {0.054529040582322*ln(x) + 0.001712639620561};
\addlegendentry{\footnotesize $K_1(T)$}

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
  width = 0.45\linewidth,
  xmin = 0, xmax = 10000,
  ymin = 0,
  xtick={2000,4000,6000,8000,10000},
  xticklabels={$2$,$4$,$6$,$8$,$10$},
  xtick scale label code/.code={$\times 10^4$},
  xlabel={$T$},
  ylabel={$\reg(T)$},
  legend pos=south east,
]

\addplot[
	black,
	only marks,
	mark = triangle*,
	mark options={rotate=60,scale=0.8,fill=gray},]
  table {UCB2.dat};
\addlegendentry{\footnotesize UCB}

\addplot[
	black,
	only marks,
	mark = triangle*,
	mark options={scale=0.8,fill=gray},]
  table {LCB2.dat};
\addlegendentry{\footnotesize LCB}

\addplot[
	smooth,
  solid,
  color=blue,
  samples=1000,
  domain=3:10000,
  ]
  {1.044085633616958*x^(2/3) -12.378853078476030};
\addlegendentry{\footnotesize $K_2(T)$}

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
  width = 0.45\linewidth,
  xmin = 0, xmax = 10000,
  ymin = 0,
  xtick={2000,4000,6000,8000,10000},
  xticklabels={$2$,$4$,$6$,$8$,$10$},
  xtick scale label code/.code={$\times 10^4$},
  xlabel={$T$},
  ylabel={$\reg(T)$},
  legend pos=south east,
]

\addplot[
	black,
	only marks,
	mark = triangle*,
	mark options={rotate=60,scale=0.8,fill=gray},]
  table {UCB3.dat};
\addlegendentry{\footnotesize UCB}

\addplot[
	black,
	only marks,
	mark = triangle*,
	mark options={scale=0.8,fill=gray},]
  table {LCB3.dat};
\addlegendentry{\footnotesize LCB}

\addplot[
	smooth,
  solid,
  color=blue,
  samples=1000,
  domain=3:10000,
  ]
  {0.116504722191015*x^(2/3) -0.730895188361662};
\addlegendentry{\footnotesize $K_2(T)$}

\end{axis}
\end{tikzpicture}
\caption{The triangles show the 99\% upper confidence bound (UCB) and lower confidence bound (LCB) of the mean cumulative regret for SAP (first panel), DUCB (second panel) and ADUCB (third panel), based on $100$ simulations. The blue line shows the curves $K_1$ with $\gamma_1 = 0.0545$ and $\gamma_2 = 0.00171$, $K_2$ with $\gamma_1 = 1.04$ and $\gamma_2 = -12.4$ and $K_2$ with $\gamma_1 = 0.117$ and $\gamma_2 = -0.731$.}
\label{fig:regression}
\end{center}
\end{figure}


